Vortex supercurrent inversion by frequency-symmetry conversion of Cooper pairs

We theoretically demonstrate that the vortex supercurrent can be reversed by odd-frequency Cooper pairs accompanied by surface Andreev bound states. The surface of a three-dimensional superconductor pierced by a flux quantum is considered. We compare the vortex supercurrents near the surface of the spin-singlet $s$-wave and spin-triplet $p_z$-wave superconductors using quasiclassical Eilenberger theory, where the surface is perpendicular to the $z$ direction. We demonstrate that the vortex supercurrent near the surface of a $p_z$-wave superconductor is reversed compared to those far from the surface, whereas that of an $s$-wave superconductor is not. The splitting of the zero-energy states caused by the interference of the surface Andreev bound states and Caroli-de Gennes-Matricon modes is demonstrated.

==> sup05.tex <==

\section{Maxwell equation, Riccati parametrization, and boundary conditions}\label{sec:form}

In this section, we introduce the formulations of the vector
potential, Riccati parametrization, and boundary conditions.
Under the rotational symmetry around the $z$ axis, the magnetic field $\bs{B}$ and vector
potential $\bs{A}$ are obtained from $\bs{j}$ as 
\begin{align}
	\bs{B}(\bs{r})&=\frac{1}{c}\int
  \bs{j}(\bs{r}^\prime)\times
  \frac{\bs{r}-\bs{r}^\prime}{\left|\bs{r}-\bs{r}^\prime\right|^3}
	dV^\prime,\label{B_form}\\
	\bs{A}(\bs{r})&=
	\bs{e}_\Theta\int_z^{\infty}B_\rho(\rho,z^\prime)dz^\prime
	\notag\\
	& \hspace{6mm}+\bs{e}_\Theta\frac{1}{\rho}\int_{0}^\rho\rho^\prime B_z(\rho^\prime,z=\infty)d\rho^\prime.\label{A_form}
\end{align}
We introduce a dimensionless Maxwell equation \eqref{maxeq} for numerical
calculations:
\begin{align}
	\bs{\nabla}^\prime \times 
	\left(\bs{\nabla}^\prime\times\bs{A}^\prime\right)=\frac{6}{\kappa^2}\bs{j}^\prime,
	\label{maxeq_kappa}
\end{align}
where $\bs{\nabla}'= \xi\bs{\nabla}$, $\bs{A}$ and $\bs{j}$ are normalized as 
$\bs{A}^\prime=(2\pi\xi/\Phi_0)\bs{A}$ 
and $\bs{j}^\prime=\bs{j}/j_0$ with $\Phi_0=\pi \hbar c/|e|$ and $j_0=4\pi N_0|e|v_FT_c$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In order to solve the Eilenberger equation~\eqref{eilenberger}
numerically, we
introduce the coherence function\cite{schopohl_PRB_1995,
schopohl1998transformation} $\gamma$ as
\begin{align}
	g&=\frac{1-s_\mu\gamma\ut{\gamma}}{1+s_\mu\gamma\ut{\gamma}},\quad
	f=\frac{2\gamma}{1+s_\mu\gamma\ut{\gamma}}.\label{coh_fun}
\end{align}
Substituting Eq.~\eqref{coh_fun} into Eq.~\eqref{eilenberger}, we obtain the 
Riccati-type differential equations:
\begin{align}
	\hbar\bs{v}_F\cdot \bs{\nabla} \gamma-
	2\left(\omega_n-\frac{ie}{c}\bs{v}_F\cdot\bs{A}\right)
	\gamma-\Delta+\Delta^*\gamma^2=0,\label{riccati}\\
	\hbar\bs{v}_F\cdot \bs{\nabla} \ut{\gamma}+
	2\left(\omega_n-\frac{ie}{c}\bs{v}_F\cdot\bs{A}\right)
	\ut{\gamma}+s_\mu\Delta^*-s_\mu\Delta\ut{\gamma}^2=0.\label{ut_riccati}
\end{align}
The solutions of Eq.~\eqref{eilenberger} are
given by solving Eq.~\eqref{riccati} and \eqref{ut_riccati} along the quasiclassical paths and substituting the obtained $\gamma$ and $\ut{\gamma}$ into Eq.~\eqref{coh_fun}.
We solve Eqs.~\eqref{gapeq}, \eqref{A_form}, \eqref{riccati} and
\eqref{ut_riccati} numerically in a self-consistent manner. 
The coherence functions $\gamma$ and $\ut{\gamma}$ in the
homogeneous limit
(i.e., $\nabla\cdot\gamma=0$) are given by
\begin{align}
	\gamma&=\frac{\Delta_\infty}{\omega_n+\mathrm{sign}(\omega_n)\sqrt{\omega_n^2+|\Delta_\infty|^2}},\label{coh_fun_bulk1}\\
	\ut{\gamma}&=\frac{s_\mu\Delta_\infty^*}{\omega_n+\mathrm{sign}(\omega_n)\sqrt{\omega_n^2+|\Delta_\infty|^2}},\label{coh_fun_bulk2}
\end{align}
where $\Delta_\infty$ is the bulk value of $\Delta$.

We impose the boundary conditions on the coherence
functions. 
(I) The coherence functions are equal to the values in
Eqs.~\eqref{coh_fun_bulk1} and \eqref{coh_fun_bulk2} 
deep inside the SC (i.e., $\rho\gg\xi,~z\gg\xi$).
(II) At the surface (i.e., $z=0$), we impose
\begin{align}
	\gamma(\hat{\bs{k}}_{\parallel},\hat{\bs{k}}_{z},\bs{r}_{\parallel},z=0,\omega_n)=\gamma(\hat{\bs{k}}_{\parallel},-\hat{\bs{k}}_{z},\bs{r}_{\parallel},z=0,\omega_n),\label{bc}
\end{align}
which means the specular reflection
where $\bs{r}_{\parallel}=(x,y)$.
As a result of Eq.~\eqref{bc}, 
the pair amplitude $f$ is forced to be an even
function with respects to the $k_z$ inversion at the surface.

\begin{figure}[tb]
	\includegraphics[width=\linewidth]{GF.pdf}
	\caption{Spatial dependences of 
		$|\Delta|$ in the (a) $s$-wave and (b) $p_z$-wave SCs.
	The pair potential is normalized by
	its bulk value.
	The parameters are set to $T/T_c=0.2$, $\Omega_{c}=40k_BT_c$ and $\kappa_{GL}=6\sqrt{6}$.  }
	\label{gap}
\end{figure}
\begin{figure}[tb]
	\centering
	\includegraphics[width=0.48\textwidth]{ldos_sw.pdf}
	\caption{Contour plots of the LDOS
	at (a) surface and (b) vortex core in the $s$-wave SC.
	The parameters are the same as in Fig.~\ref{gap}.
	The smearing factor is $\delta=0.005$.}
	\label{ldos_s}
\end{figure}

\section{Additional numerical results } \label{sec:num_res}
%\buf{for$s$-wave superconductor} 



In this section, we show the spatial dependence of the pair potential 
and local density of state (LDOS) for the $s$-wave SC.
We show the spatial dependences of the pair
potential in Fig.~\ref{gap}. 
As show in Fig.~\ref{gap}(a), the pair potential in
the $s$-wave SC is
suppressed near the vortex core but not at the surface. 
On the other hand, the pair function in the $p_z$-wave SC
disappears at the
vortex core and the surface as shown in Fig.~\ref{gap}(b).

In Fig.~\ref{ldos_s}, we show the LDOS in the $s$-wave SC. 
Figures~\ref{ldos_s}(a) and (b) show the LDOS at the
surface and vortex core.
In Fig.~\ref{ldos_s}, there exist sub-gap bound states near the core
known as the Caroli-de-Gennes-Matricon (CdGM) modes. 
The approximate energy dispersion of the CdGM modes have been derived 
as $E_n\simeq (n-1/2)\Delta_\infty^2/E_F$ in Ref.~\onlinecite{caroli_PL_1964}, where the half integer $(n-1/2)$ is the quantum number of the angular momentum.
The eigenfunction of the CdGM mode labeled by $n$ has 
a maximum amplitude at a radius distance of the order $\rho\simeq (n-1/2)/k_F$\cite{gygi_PRB_1991}.
Thus, the evolution of sub-gap states in Fig.~\ref{ldos_s}(a)
corresponds to the dispersion relation 
of the CdGM modes.

\section{Renormalized spherical harmonics}\label{sec:sphe_harm}
We use the real spherical harmonics $Y_{lm}$ to analyze
the pair amplitudes. 
We abbreviate the expansion coefficients $f_{lm}$ in the main texts for simplicity.
We summarize $Y_{lm}$ and the notation of $f_{lm}$ in Table \ref{table:fnotation}.
The spherical harmonics
$Y_{lm}$ is normalized to satisfy the orthonormal relation
\begin{align}
	\int Y_{lm}Y_{l^\prime m^\prime}d\Omega=\delta_{ll^\prime}\delta_{mm^\prime},
\end{align}
where $d\Omega=\sin\theta d\phi d\theta$.

%In addition to this condition, we chose \dots
%\begin{align}
%  \tilde{Y}_0^0 &= 1, ~ ~
%  \tilde{Y}_1^0 = k_z, ~ ~
%  \tilde{Y}_1^{\pm 1} = k_x \pm i k_y, \\
%	%
%  \tilde{Y}_2^{0}    &= (3k_z^2-1     )/2, ~ ~
%  \tilde{Y}_2^{\pm 1} = 2(k_x \pm i k_y)k_z, ~ ~
%  \tilde{Y}_2^{\pm 2} = (k_x \pm i k_y)^2, \\
%	%
%  \tilde{Y}_3^{0}    &= \frac{1}{2}(5k_z^3-3k_z), ~ ~
%  \tilde{Y}_3^{\pm 1} = \frac{\sqrt{135}}{16}(k_x \pm i k_y) (5k_z^2-1), ~ ~
%  \tilde{Y}_3^{\pm 2} = \frac{\sqrt{27}}{2}(k_x \pm i k_y)^2 k_z, ~ ~
%  \tilde{Y}_3^{\pm 3} = (k_x \pm i k_y)^3, 
%  \label{}
%\end{align}
%The pre-factors are decided such that $\mathrm{max}[Y_l^m]=1$ on the
%Fermi sphere. The norms of them are no longer normalized. The norms
%are given as following: 
%\begin{align}
%  \langle \tilde{Y}_0^0|\tilde{Y}_0^0\rangle&= 1, ~ ~
%  \langle \tilde{Y}_1^{    0}|\tilde{Y}_1^{    0} \rangle = \frac{1}{3}, ~ ~
%  \langle \tilde{Y}_1^{\pm 1}|\tilde{Y}_1^{\pm 1} \rangle = \frac{2}{3}, \\
%	%
%  \langle \tilde{Y}_2^0      |\tilde{Y}_2^0       \rangle&= \frac{1}{5}, ~ ~
%  \langle \tilde{Y}_2^{\pm 1}|\tilde{Y}_2^{\pm 1} \rangle = \frac{8}{5}, ~ ~
%  \langle \tilde{Y}_2^{\pm 2}|\tilde{Y}_2^{\pm 2} \rangle = \frac{8}{15}, \\
%	%
%  \langle \tilde{Y}_3^0      |\tilde{Y}_3^0       \rangle&= \frac{1}{7}, ~ ~
%  \langle \tilde{Y}_3^{\pm 1}|\tilde{Y}_3^{\pm 1} \rangle = \frac{45}{112}, ~ ~
%  \langle \tilde{Y}_3^{\pm 2}|\tilde{Y}_3^{\pm 2} \rangle = \frac{18}{35}, ~ ~
%  \langle \tilde{Y}_3^{\pm 3}|\tilde{Y}_3^{\pm 3} \rangle = \frac{16}{35}, \\
%\label{}
%\end{align}
%
%The expansion coefficients $f_{lm}$ of the pair amplitude with respect to the real spherical harmonics is denoted according to Table \ref{table:fnotation} for simplicity.



\begin{table*}[tb]
	\caption{Notation of the expansion coefficients $f_{lm}$}
  \label{table:fnotation}
  \centering
  %\begin{tabular}{crlcl}
  %  \hline
  %  ~ $l$ & ~ ~$m$~ ~ & Atomic orbital & Real spherical harmonics $Y_{lm}$ & Notation of $f_{lm}$ \\
  %  \hline \hline
  %  $0$ & $ 0$ & $s              $ & $\sqrt{({1}  /{ 4\pi})}$                                         & $f_{0}          $ \\[3mm]
  %  $1$ & $-1$ & $p_y            $ & $\sqrt{({3}  /{ 4\pi})}\sin\phi\sin\theta$                       & $f_{y}          $ \\[1mm]
  %  ~~~ & $ 0$ & $p_z            $ & $\sqrt{({3}  /{ 4\pi})}\cos\theta$                               & $f_{z}          $ \\[1mm]
  %  ~~~ & $ 1$ & $p_x            $ & $\sqrt{({3}  /{ 4\pi})}\cos\phi\sin\theta$                       & $f_{x}          $ \\[3mm]
  %  $2$ & $-2$ & $d_{xy}         $ & $\sqrt{({15} /{16\pi})}\sin2\phi\sin^2\theta$                    & $f_{xy }        $ \\[1mm]
  %  ~~~ & $-1$ & $d_{yz}         $ & $\sqrt{({15} /{16\pi})}\sin\phi\sin2\theta$                      & $f_{yz }        $ \\[1mm]
  %  ~~~ & $ 0$ & $d_{z^2}        $ & $\sqrt{({5}  /{16\pi})}\left(3\cos^2\theta-1\right)$             & $f_{z^2}        $ \\[1mm]
  %  ~~~ & $ 1$ & $d_{xz}         $ & $\sqrt{({15} /{16\pi})}\cos\phi\sin2\theta$                      & $f_{xz }        $ \\[1mm]
  %  ~~~ & $ 2$ & $d_{x^2-y^2}    $ & $\sqrt{({15} /{16\pi})}\cos2\phi\sin^2\theta$                    & $f_{x^2-y^2}    $ \\[3mm]
  %  $3$ & $-3$ & $f_{y(3x^2-y^2)}$ & $\sqrt{({35} /{32\pi})}\sin3\phi\sin^3\theta$                    & $f_{y(3x^2-y^2)}$ \\[1mm]
  %  ~~~ & $-2$ & $f_{xyz}        $ & $\sqrt{({105}/{16\pi})}\sin2\phi\sin^2\theta\cos\theta$          & $f_{xyz}        $ \\[1mm]
  %  ~~~ & $-1$ & $f_{yz^2}       $ & $\sqrt{({21} /{32\pi})}\sin\phi\sin\theta\left(5\cos^2-1\right)$ & $f_{yz^2}       $ \\[1mm]
  %  ~~~ & $ 0$ & $f_{z^3}        $ & $\sqrt{({7}  /{16\pi})}\left(5\cos^3\theta-3\cos\theta\right)$   & $f_{z^3}        $ \\[1mm]
  %  ~~~ & $ 1$ & $f_{xz^2}       $ & $\sqrt{({21} /{32\pi})}\cos\phi\sin\theta\left(5\cos^2-1\right)$ & $f_{xz^2}       $ \\[1mm]
  %  ~~~ & $ 2$ & $f_{z(x^2-y^2)} $ & $\sqrt{({105}/{16\pi})}\cos2\phi\sin^2\theta\cos\theta$          & $f_{z(x^2-y^2)} $ \\[1mm]
  %  ~~~ & $ 3$ & $f_{x(x^2-3y^2)}$ & $\sqrt{({35} /{32\pi})}\cos3\phi\sin^3\theta$                    & $f_{x(x^2-3y^2)}$ \\[1mm]
  %  \hline
  %\end{tabular}
	\includegraphics[width=0.7\textwidth]{table.pdf}
\end{table*}



















\section{Vortex supercurrent and frequency symmetry of Cooper pairs} \label{sec:ConvFreq}

The direction of the vortex supercurrent is related to the frequency
symmetry of Cooper pairs. 
The azimuthal component of the current density \eqref{jeq} is
\begin{align}
	& j_\Phi(\bs{r})
	= -j_0%{4\pi N_0ev_F T_c} 
	\frac{T}{T_c}
	\sum_{n=0}^{N_{\mathrm{c}}}
	\int\frac{d\Omega}{4\pi}
	\sin\theta\sin\phi\mathrm{Im}g(\hat{\bs{k}},\bs{r},\omega_n), 
\end{align}
where $j_0={4\pi N_0|e|v_F T_c} $.
Namely, the direction of the current is determined by the sign of 
$\mathrm{Im}[g]$. 
Using the normalization condition for the quasiclassical Green's
function (i.e., $g^2=1-s_\mu f\ut{f}$), we have 
\begin{align}
	& g=\sqrt{1-|f_e|^2+|f_o|^2-2i\mathrm{Im}f_of_e^*}, 
	\label{eq:g}
	\\
	%
	& f_{e(o)} = \frac{1}{2}[f(\bs{r}, \bs{k}, \omega) +(-) f(\bs{r}, \bs{k}, -\omega)], 
\end{align}
where $f_e$ and $f_o$ represent respectively the even- and odd-frequency
component, and we have used the symmetry relation between $f$ and $\ut{f}$
[i.e., $\ut{f}(\bs{r}, \bs{k}, \omega)=f^*(\bs{r},-\bs{k}, \omega)$].

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.46\textwidth]{pair_amp_fig.pdf}
	\caption{Schematic picture of the spatial distribution of the pair
	amplitudes around the vortex in the $p_z$-wave SC.  The even and
	odd-$\omega$ pairs are dominant near the vortex core at the surface
  and deep inside the SC.}
	\label{pair_amp}
\end{figure}

We analyze the direction of the vortex supercurrent in the vicinity of
the vortex core. From Fig.~\ref{pair_amp}, deep inside
the SC, the pair amplitudes around the vortex core can be approximated
as 
\begin{align}
	f_e \approx \rho F, \quad 
	f_o \approx -RF e^{-i\phi},
	\label{eq:even-odd}
\end{align}
where $F=F(\hat{\bs{k}})$ and we have introduced the constant $R$
($0<R<1$) that expresses the relative amplitude of $f_o$ to $f_e$. 
The subdominant component has an additional phase factor ($-e^{-i\phi}$)
from the phase winding of the vortex. 
%
Substituting Eq.~\eqref{eq:even-odd} into Eq.~\eqref{eq:g}, we have
\begin{align}
	g&=\sqrt{1-\rho^2|F|^2+R^2|F|^2+2i\rho R|F|^2\mathrm{Im}e^{-i\phi}}\\
   &=\sqrt{1+R^2|F|^2}
	 -i\rho\frac{R|F|^2\sin\phi}{\sqrt{1+R^2|F|^2}}
	 +O(\rho^2)
\end{align}
with $\rho \ll \xi$. 
The equation above results in 
\begin{align}
  -j_0\sin\phi\mathrm{Im}g
	=
	\rho\frac{j_0R|F|^2\sin^2\phi}{\sqrt{1+R^2|F|^2}}+O(\rho^2), 
	\label{eq:cur_dir1}
\end{align}
meaning that the electric current flows in the opposite direction of
the phase winding $e^{-i\Phi}$ around the vortex core (i.e., $j_\Phi >0$). 

At the surface of a $p_z$-wave SC, the symmetry conversion occurs
because of the ABSs. The pair amplitudes can be expressed as 
\begin{align}
	f_e=-RF e^{-i\phi},\quad f_o=\rho F, %\quad 0<C<1,\quad 
	\label{eq:even-odd2}
\end{align}
where we can show $R^2|F|^2=1$ by solving the Riccati-type differential equations \eqref{riccatieq} at $T=0$ and $\rho=0$. 
	We assume $f_e$ near the core has the maximum value at $\omega_n=0$.
	From this assumption, we obtain $R^2|F|^2<1$ at finite matsubara frequencies.
Substituting Eq.~\eqref{eq:even-odd2} into Eq.~\eqref{eq:g}, we have
\begin{align}
	g&=\sqrt{1-R^2|F|^2+\rho^2|F|^2+2i\rho R|F|^2\mathrm{Im}e^{i\phi}}
       \\&=\sqrt{1-R^2|F|^2}
			 +i\rho\frac{R|F|^2\sin\phi}{\sqrt{1-R^2|F|^2}}+O(\rho^2). 
\end{align}
Therefore, the direction of the current density is given by 
\begin{align}
  -j_0\sin\phi\mathrm{Im}[g]
	=-\rho\frac{j_0R|F|^2\sin^2\phi}{\sqrt{1-R^2|F|^2}}+O(\rho^2)
	\label{eq:cur_dir2}
\end{align}
Comparing Eqs.~\eqref{eq:cur_dir1} and \eqref{eq:cur_dir2}, we see
that the frequency-symmetry conversion results in the vortex-current inversion. 


\section{Analytical Calculations by Kramer-Pesch approximation} \label{sec:kp_app}
\begin{figure}[tb]
	\centering
	\includegraphics[width=0.2\textwidth]{sys_trans.pdf}
\caption{Coordinate transformation from $(x,y,z)$ to $(a,b,z)$.}
	\label{fig_cotr}
\end{figure}

In this section, we analytically calculate the quasi-classical Green's
functions by the Kramer-Pesch approximation
\cite{kramer_ZP_1974,nagai_JPSJ_2006, nagai_JPSJ_2019} and
reproduce two
numerical results, the reversal of the vortex current 
and suppression of the LDOS at the intersection point 
of the surface and vortex core, for more general SCs.  
In the Kramer-Pesch approximation, we obtain the solutions of the Riccati-type differential equations up to
the first order of the displacement $b$ from the vortex core and Matsubara frequency $\omega_n$.
Thus, the Kramer-Pesch approximation is appropriate near the vortex core
$\rho\ll\xi$ and in low temperature $k_BT\ll|\Delta|$.
In this section, We follow the
method in Ref.~\onlinecite{nagai_JPSJ_2006}.

We start with the Riccati-type differential equations with $\bs{A}=0$:
\begin{align}
	\bs{v}_F\cdot\nabla\gamma+2\omega_n\gamma-\Delta+\Delta^*\gamma^2=0,\label{riccatieq}\\
  \bs{v}_F\cdot\nabla\ut{\gamma}-2\omega_n\ut{\gamma}+s_\mu\Delta^*-s_\mu\Delta\ut{\gamma}^2=0,
\end{align}
where we use the units $\hbar=k_B=1$.
We introduce the coordinate transformation as in Fig.\ref{fig_cotr}:
\begin{align}
  a&=x\cos\phi+y\sin\phi,\\
	b&=-x\sin\phi+y\cos\phi, 
\end{align}
where the angle $\phi$ characterizes the direction of the
momentum: $\hat{\bs{k}} = (\sin\theta\cos\phi, \sin\theta\sin\phi,
\cos\theta)$. The
$b$-axis is perpendicular to
the projected momentum
$\bs{k}_{\parallel}=(\sin\theta\cos\phi,\sin\theta\sin\phi,0)$.
%
We solve the Riccati-type differential equations by integrating
$\gamma$ or $\ut{\gamma}$ in the direction $\hat{\bs{k}}$.  The
impact parameter $b$ is
constant on the integrating path and corresponds to the distance
between the integrating path and 
vortex core. 
In this coordinate $\bs{r}=(a,b,z)$, the Riccati-type
differential equations are rewritten as
\begin{align}
  & v_F\left\{\sin\theta\frac{\partial}{\partial a}
	+\cos\theta\frac{\partial}{\partial z}\right\}\gamma
	+2\omega_n\gamma-\Delta+\Delta^*\gamma^2=0,\\
	%
  & v_F\left\{\sin\theta\frac{\partial}{\partial a}
	+\cos\theta\frac{\partial}{\partial z}\right\}\ut{\gamma}
	-2\omega_n\ut{\gamma}+s_\mu\Delta^*-s_\mu\Delta\ut{\gamma}^2=0.
\end{align}
In the
analytic calculation, the pair potential is written in more general
form: 
\begin{align}
  \Delta(\hat{\bs{k}})&=h(\rho,z)e^{-i\Phi}\Psi(\hat{\bs{k}}).
\end{align}
where the real function $h$ and the complex function $\Psi$
describe the spatial and momentum dependence of $\Delta$. In
addition, we assume that $\Psi$ satisfies
$s_\theta=\Psi(\theta,\phi)/\Psi(\pi-\theta,\phi)=\pm1$.  In the case
of $s_\theta=1$ and $-1$, the ABSs is absence and present on the
surface perpendicular to the $z$ axis. 
We expand the pair potential as
\begin{align}
  & \Delta(\hat{\bs{k}},\bs{r})=\Delta_0+\Delta_1,\\
  & \Delta_0=h(|a|,z)e^{-i\phi}\mathrm{sign}(a)\Psi(\hat{\bs{k}}),\\
  & \Delta_1=-h(|a|,z)e^{-i\phi}\mathrm{sign}(a)i\frac{b}{a}\Psi(\hat{\bs{k}}),
\end{align}
with respect to $b$.
The solutions \eqref{coh_fun_bulk1} and \eqref{coh_fun_bulk2} in the homogeneous limit are also expanded in terms of 
$b$ and $\omega_n$ as
\begin{widetext}
\begin{align}
  \gamma(\bs{r},\hat{\bs{k}},\omega_n)&=\mathrm{sign}(a\omega_n)\left\{\frac{\Psi(\hat{\bs{k}})e^{-i\phi}}{|\Psi(\hat{\bs{k}})|}-\frac{\Psi(\hat{\bs{k}})e^{-i\phi}}{h(|a|,z)|\Psi(\hat{\bs{k}})|^2}|\omega_n|-i\frac{\Psi(\hat{\bs{k}})e^{-i\phi}}{|\Psi(\hat{\bs{k}})|}\frac{b}{a}\right\}+\cdots,\\
  \ut{\gamma}(\bs{r},\hat{\bs{k}},\omega_n)&=\mathrm{sign}(a\omega_n)\left\{\frac{s_\mu\Psi^*(\hat{\bs{k}})e^{i\phi}}{|\Psi(\hat{\bs{k}})|}-\frac{s_\mu\Psi^*(\hat{\bs{k}})e^{i\phi}}{h(|a|,z)|\Psi(\hat{\bs{k}})|^2}|\omega_n|+i\frac{s_\mu\Psi^*(\hat{\bs{k}})e^{i\phi}}{|\Psi(\hat{\bs{k}})|}\frac{b}{a}\right\}+\cdots.
\end{align}
When we set the cut-off of the integral path as $a_c>0$, the boundary conditions (I) in the Appendix \ref{sec:form} are given as
\begin{align}
	\gamma(a=-a_c,\frac{\pi}{2}<\theta\le\pi,\omega_n>0)&=-\frac{\Psi(\hat{\bs{k}})e^{-i\phi}}{|\Psi(\hat{\bs{k}})|}+\frac{\Psi(\hat{\bs{k}})e^{-i\phi}}{\Delta_0|\Psi(\hat{\bs{k}})|^2}|\omega_n|-i\frac{\Psi(\hat{\bs{k}})e^{-i\phi}}{|\Psi(\hat{\bs{k}})|}\frac{b}{a_c},\label{bc1}\\
  \ut{\gamma}(a=a_c,0\le\theta<\frac{\pi}{2},\omega_n>0)&=\frac{s_\mu\Psi^*(\hat{\bs{k}})e^{i\phi}}{|\Psi(\hat{\bs{k}})|}-\frac{s_\mu\Psi^*(\hat{\bs{k}})e^{i\phi}}{\Delta_0|\Psi(\hat{\bs{k}})|^2}|\omega_n|+i\frac{s_\mu\Psi^*(\hat{\bs{k}})e^{i\phi}}{|\Psi(\hat{\bs{k}})|}\frac{b}{a_c},\label{bc2}
\end{align}
The Riccati-type differential equations of the zeroth order 
of $b$ and $\omega_n$ are written as
\begin{align}
  v_F\left\{\sin\theta\frac{\partial}{\partial a}+\cos\theta\frac{\partial}{\partial z}\right\}\gamma_0-\Delta_0+\Delta^*_0\gamma_0^2=0,\\
  v_F\left\{\sin\theta\frac{\partial}{\partial a}+\cos\theta\frac{\partial}{\partial z}\right\}\ut{\gamma}_0+s_\mu\Delta^*_0-s_\mu\Delta_0\ut{\gamma}^2_0=0.
\end{align}
The solutions of these equations are given by
\begin{align}
\gamma_0(\hat{\bs{k}},\omega_n>0)&
=-\frac{\Psi(\mathrm{max}\{\theta,\pi-\theta\},\phi)}{|\Psi(\hat{\bs{k}})|}e^{-i\phi},\\
\ut{\gamma}_0(\hat{\bs{k}},\omega_n>0)&
=\frac{s_\mu\Psi^*(\mathrm{min}\{\theta,\pi-\theta\},\phi)}{|\Psi(\hat{\bs{k}})|}e^{i\phi},
\end{align}
which satisfies the boundary conditions 
 \eqref{bc}, \eqref{bc1} and \eqref{bc2}.
The first order Riccati-type differential equations are written as
\begin{align}
  v_F\left\{\sin\theta\frac{\partial}{\partial a}+\cos\theta\frac{\partial}{\partial z}\right\}\gamma_1+2\omega_n\gamma_0-\Delta_1+2\Delta^*_0\gamma_0\gamma_1+\Delta_1^*\gamma_0^2=0,\\
  v_F\left\{\sin\theta\frac{\partial}{\partial a}+\cos\theta\frac{\partial}{\partial z}\right\}\ut{\gamma}_1-2\omega_n\ut{\gamma}_0+s_\mu\Delta_1^*-2s_\mu\Delta_0\ut{\gamma}_0\ut{\gamma}_1-s_\mu\Delta_1\ut{\gamma}_0^2=0.
\end{align}
The general solutions of these equations are given as
\begin{align}
	\gamma_1&=\frac{2}{v_F}\exp\left[2|\Psi(\hat{\bs{k}})|F(\sigma,z_0,\theta)\right]\int^\sigma_{\sigma_0}d\sigma^\prime\left[-i\frac{b}{\sigma^\prime\sin\theta}\Delta_0-\omega_n\gamma_0\right]\exp\left[-2|\Psi(\hat{\bs{k}})|F(\sigma^\prime,z_0,\theta)\right]\\&+C_0\exp\left[2|\Psi(\hat{\bs{k}})|F(\sigma,z_0,\theta)\right],\\
  \ut{\gamma}_1&=\frac{2}{v_F}\exp\left[2s_\theta|\Psi(\hat{\bs{k}})|F(\sigma,z_0,\theta)\right]\int^\sigma_{\ut{\sigma}_0}d\sigma^\prime\left[-is_\mu\frac{b}{\sigma^\prime\sin\theta}\Delta^*_0+\omega_n\ut{\gamma}_0\right]\exp\left[-2s_\theta|\Psi(\hat{\bs{k}})|F(\sigma^\prime,z_0,\theta)\right]\\&+\ut{C}_0\exp\left[2s_\theta|\Psi(\hat{\bs{k}})|F(\sigma,z_0,\theta)\right],\\
  F&(\sigma,z_0,\theta)=\int_{-\frac{z_0}{\cos\theta}}^\sigma\mathrm{sign}(\sigma^\prime)\frac{\Psi(\max\{\theta,\pi-\theta\},\phi)}{\Psi(\bs{k})}h(|\sigma^\prime|\sin\theta,\sigma^\prime\cos\theta+z_0)d\sigma^\prime,\\
  a&=\sigma\sin\theta,\\
  z&=\sigma\cos\theta+z_0
\end{align}
where $\sigma_0, C_0,\ut{\sigma}_0$ and $\ut{C}_0$ are integral constants.
In $\pi/2<\theta\le\pi$, we obtain the first order coherence function
$\gamma_1$ from the boundary condition \eqref{bc1} as  
\begin{align}
  \gamma_1&=\frac{2}{v_F}\exp\left[2|\Psi(\hat{\bs{k}})|F(\sigma,z_0,\theta)\right]\int^\sigma_{-\frac{a_c}{\sin\theta}}d\sigma^\prime\left[-i\frac{b}{\sigma^\prime\sin\theta}\Delta_0-\omega_n\gamma_0\right]\exp\left[-2|\Psi(\hat{\bs{k}})|F(\sigma^\prime,z_0,\theta)\right]
        \\&+\left\{\frac{\Psi(\hat{\bs{k}})e^{-i\phi}}{\Delta_\infty|\Psi(\hat{\bs{k}})|^2}|\omega_n|-i\frac{\Psi(\hat{\bs{k}})e^{-i\phi}}{|\Psi(\hat{\bs{k}})|}\frac{b}{a_c}\right\}\exp\left[2|\Psi(\hat{\bs{k}})|\left\{F(\sigma,z_0,\theta)-F\left(-\frac{a_c}{\sin\theta},z_0,\theta\right)\right\}\right].
\end{align}
The other function $\ut{\gamma}_1$ in $0\le\theta<\pi/2$ is given from the boundary condition
\eqref{bc2} as 
\begin{align}
  \ut{\gamma}_1&=-\frac{2}{v_F}\exp\left[2s_\theta|\Psi(\hat{\bs{k}})|F(\sigma,z_0,\theta)\right]\int_\sigma^{\frac{a_c}{\sin\theta}}d\sigma^\prime\left[-is_\mu\frac{b}{\sigma^\prime\sin\theta}\Delta^*_0+\omega_n\ut{\gamma}_0\right]\exp\left[-2s_\theta|\Psi(\hat{\bs{k}})|F(\sigma^\prime,z_0,\theta)\right]
                     \\&-\left\{\frac{s_\mu\Psi^*(\hat{\bs{k}})e^{i\phi}}{\Delta_\infty|\Psi(\hat{\bs{k}})|^2}|\omega_n|-i\frac{s_\mu\Psi^*(\hat{\bs{k}})e^{i\phi}}{|\Psi(\hat{\bs{k}})|}\frac{b}{a_c}\right\}\exp\left[2s_\theta|\Psi(\hat{\bs{k}})|\left\{F(\sigma,z_0,\theta)-F\left(\frac{a_c}{\sin\theta},z_0,\theta\right)\right\}\right].
\end{align}
We respectively set the integral constants as $\sigma_0=-a_c/\sin\theta$ and $\ut{\sigma}_0=a_c/\sin\theta$.
From the boundary condition \eqref{bc}, $\gamma_1$ in $0\le\theta<\pi/2$ and $\ut{\gamma}_1$ in $\pi/2<\theta\le\pi$ are given as
\begin{align}
  \gamma_1&=\frac{2}{v_F}\exp\left[2|\Psi(\hat{\bs{k}})|F(\sigma,z_0,\theta)\right]\int^\sigma_{-\frac{z_0}{\cos\theta}}d\sigma^\prime\left[-i\frac{b}{\sigma^\prime\sin\theta}\Delta_0-\omega_n\gamma_0\right]\exp\left[-2|\Psi(\hat{\bs{k}})|F(\sigma^\prime,z_0,\theta)\right]\\
          &+\frac{2}{v_F}\int^{-\frac{z_0}{\cos\theta}}_{-\frac{a_c}{\sin\theta}}d\sigma^\prime\left[-i\frac{b}{\sigma^\prime\sin\theta}\Delta_0(-z_0,\pi-\theta)-\omega_n\gamma_0\right]\exp\left[2|\Psi(\hat{\bs{k}})|\left\{F(\sigma,z_0,\theta)-F(\sigma^\prime,-z_0,\pi-\theta)\right\}\right]
        \\&+s_\theta\left\{\frac{\Psi(\hat{\bs{k}})e^{-i\phi}}{\Delta_\infty|\Psi(\hat{\bs{k}})|^2}|\omega_n|-i\frac{\Psi(\hat{\bs{k}})e^{-i\phi}}{|\Psi(\hat{\bs{k}})|}\frac{b}{a_c}\right\}\exp\left[2|\Psi(\hat{\bs{k}})|\left\{F(\sigma,z_0,\theta)-F\left(-\frac{a_c}{\sin\theta},-z_0,\pi-\theta\right)\right\}\right],\\
	\ut{\gamma}_1&=-\frac{2}{v_F}\exp\left[2s_\theta|\Psi(\hat{\bs{k}})|F(\sigma,z_0,\theta)\right]\int_\sigma^{-\frac{z_0}{\cos\theta}}d\sigma^\prime\left[-is_\mu\frac{b}{\sigma^\prime\sin\theta}\Delta^*_0+\omega_n\ut{\gamma}_0\right]\exp\left[-2s_\theta|\Psi(\hat{\bs{k}})|F(\sigma^\prime,z_0,\theta)\right]
		     \\&-\frac{2}{v_F}\int_{-\frac{z_0}{\cos\theta}}^{\frac{a_c}{\sin\theta}}d\sigma^\prime\left[-is_\mu\frac{b}{\sigma^\prime\sin\theta}\Delta_0^*(-z_0,\pi-\theta)+\omega_n\ut{\gamma}_0\right]\exp\left[2s_\theta|\Psi(\bs{k})|\left\{F(\sigma,z_0,\theta)-F(\sigma^\prime,-z_0,\pi-\theta)\right\}\right]\\
                       &-s_\theta\left\{\frac{s_\mu\Psi^*(\hat{\bs{k}})e^{i\phi}}{\Delta_\infty|\Psi(\hat{\bs{k}})|^2}|\omega_n|-i\frac{s_\mu\Psi^*(\hat{\bs{k}})e^{i\phi}}{|\Psi(\hat{\bs{k}})|}\frac{b}{a_c}\right\}\exp\left[2s_\theta|\Psi(\hat{\bs{k}})|\left\{F(\sigma,z_0,\theta)-F\left(\frac{a_c}{\sin\theta},-z_0,\pi-\theta\right)\right\}\right].
\end{align}
When we take $z=0,~a_c\rightarrow\infty$, we obtain
\begin{align}
  %F(\sigma,z_0,\theta)&=s_\theta F(-\sigma,z_0,\pi-\theta),\\
  F\left(\sigma=-\frac{z_0}{\cos\theta},z_0,\theta\right)&=0,\\
  F\left(\sigma=-\infty,z_0,\frac{\pi}{2}<\theta\le\pi\right)&=s_\theta F\left(\sigma=+\infty,z_0,0\le \theta<\frac{\pi}{2}\right)=\infty.
\end{align}
As a result, $\gamma_1$ and $\ut{\gamma}_1$ in $0\le\theta<\pi/2$ is given as
\begin{align}
  \gamma_1&=\frac{2}{v_F}\int^{-\frac{z_0}{\cos\theta}}_{-\infty}d\sigma^\prime\left[-i\frac{b}{\sigma^\prime\sin\theta}\Delta_0(-z_0,\pi-\theta)-\omega_n\gamma_0\right]\exp\left[-2|\Psi(\hat{\bs{k}})|F(\sigma^\prime,-z_0,\pi-\theta)\right],\\
  \ut{\gamma}_1&=-\frac{2}{v_F}\int_{-\frac{z_0}{\cos\theta}}^{\infty}d\sigma^\prime\left[-is_\mu\frac{b}{\sigma^\prime\sin\theta}\Delta^*_0+\omega_n\ut{\gamma}_0\right]\exp\left[-2s_\theta|\Psi(\hat{\bs{k}})|F(\sigma^\prime,z_0,\theta)\right],
\end{align}
and ones in $\pi/2\le\theta<\pi$ is given as
\begin{align}
\gamma_1&=\frac{2}{v_F}\int^{-\frac{z_0}{\cos\theta}}_{-\infty}d\sigma^\prime\left[-i\frac{b}{\sigma^\prime\sin\theta}\Delta_0-\omega_n\gamma_0\right]\exp\left[-2|\Psi(\hat{\bs{k}})|F(\sigma^\prime,z_0,\theta)\right],\\
  \ut{\gamma}_1&=-\frac{2}{v_F}\int_{-\frac{z_0}{\cos\theta}}^{\infty}d\sigma^\prime\left[-is_\mu\frac{b}{\sigma^\prime\sin\theta}\Delta_0^*(-z_0,\pi-\theta)+\omega_n\ut{\gamma}_0\right]\exp\left[-2s_\theta|\Psi(\bs{k})|F(\sigma^\prime,-z_0,\pi-\theta)\right].
\end{align}
We can replace $z$ to $|z|$ due to $z=\sigma\cos\theta+z_0>0$. 
By this substitution, we can rewrite $\gamma_1$ and 
$\ut{\gamma}_1$ in $0\le\theta\le\pi$ as
\begin{align}
  \gamma_1&=\frac{2}{v_F}\int^{-\frac{z_0}{\cos\theta}}_{-\infty}d\sigma^\prime\left[-i\frac{b}{\sigma^\prime\sin\theta}\bar{\Delta}(\sigma^\prime)-\omega_n\gamma_0\right]\exp\left[-2|\Psi(\bs{k})|\bar{F}(\sigma^\prime)\right],\\
\ut{\gamma}_1&=-\frac{2}{v_F}\int_{-\frac{z_0}{\cos\theta}}^{\infty}d\sigma^\prime\left[-is_\mu s_\theta\frac{b}{\sigma^\prime\sin\theta}\bar{\Delta}^*(\sigma^\prime)+\omega_n\ut{\gamma}_0\right]\exp\left[-2|\Psi(\bs{k})|\bar{F}(\sigma^\prime)\right],
\end{align}
where we define $\bar{\Delta}$ and $\bar{F}$ as
\begin{align}
  \bar{\Delta}(\sigma,z_0,\hat{\bs{k}})&=h(|\sigma^\prime|\sin\theta,|\sigma^\prime\cos\theta+z_0|)e^{i\phi}\mathrm{sign}(\sigma)\Psi(\max\{\theta,\pi-\theta\},\phi),\\
  \bar{F}(\sigma,z_0,\hat{\bs{k}})&=\int_{-\frac{z_0}{\cos\theta}}^{\sigma}\mathrm{sign}(\sigma^{\prime})h(|\sigma^{\prime}|\sin\theta,|\sigma^{\prime}\cos\theta+z_0|)d\sigma^{\prime}.
\end{align}

The quasi-classical Green functions are expanded as
\begin{align}
  g&=\frac{1-s_\mu\gamma\ut{\gamma}}{1+s_\mu\gamma\ut{\gamma}}
  \simeq\frac{1-s_\mu\left(\gamma_0\ut{\gamma}_0+\gamma_1\ut{\gamma}_0+\gamma_0\ut{\gamma}_1\right)}{1+s_\mu\left(\gamma_0\ut{\gamma}_0+\gamma_1\ut{\gamma}_0+\gamma_0\ut{\gamma}_1\right)},\\
  f&=\frac{2\gamma}{1+s_\mu\gamma\ut{\gamma}}
  \simeq\frac{2\gamma_0+2\gamma_1}{1+s_\mu\left(\gamma_0\ut{\gamma}_0+\gamma_1\ut{\gamma}_0+\gamma_0\ut{\gamma}_1\right)}.
\end{align}
The relation $\gamma_0\ut{\gamma}_0=-s_\mu
s_\theta$ is important.
In the case of $s_\theta=1$, zeroth order Green functions diverge,
whereas ones do not in the case of $s_\theta=-1$.  
We consider the case of $s_\theta=-1$. In this case, the first order
Green functions are approximated as
\begin{align}
	g\simeq-\frac{s_\mu W}{2+s_\mu W},
	\hspace{9mm}
	f\simeq\frac{2\gamma_0+2\gamma_1}{2+s_\mu W},\label{fexpand}
\end{align}
where we define
\begin{align}
	W(b,z_0,\bs{k})&=\gamma_1\ut{\gamma}_0+\gamma_0\ut{\gamma}_1
		     =\frac{2}{v_F}\int^{\infty}_{-\infty}d\sigma^\prime\left[-i\frac{b}{\sigma^\prime\sin\theta}\bar{\Delta}(\sigma^\prime)\ut{\gamma}_0-s_\mu\omega_n\right]\exp\left[-2|\Psi(\bs{k})|\bar{F}(\sigma^\prime)\right].
\end{align}
In the cylindrical coordinate $\bs{r}=(\rho,\Phi,z=0)$, $W$ is rewritten as
\begin{align}
  W(\rho,\Phi,z=0,\bs{k})&=-2s_\mu(i\rho CD+\omega_nC),
\end{align}
where we use $b=\rho\sin(\phi-\Phi)$ and define $D$ and $C$ as
\begin{align}
  D(\rho,\Phi,\bs{k})&=\frac{2}{C(\rho,\Phi,\bs{k})}\int^{\infty}_{-\infty}d\sigma^\prime\frac{\sin(\phi-\Phi)}{\sigma^\prime\sin\theta}h\left(|\sigma|\sin\theta,\left|\sigma\cos\theta-\rho\frac{\cos(\phi-\Phi)}{\tan\theta}\right|\right)\exp\left[-2|\Psi(\bs{k})|\bar{F}(\rho,\Phi,\sigma^\prime,\bs{k})\right]\\
		  &=\frac{\sin(\phi-\Phi)}{\sin\theta}\tilde{D}(\rho,\Phi,\bs{k}),\\
  C(\rho,\Phi,\bs{k})&=\frac{2}{v_F}\int^{\infty}_{-\infty}d\sigma^\prime\exp\left[-2|\Psi(\bs{k})|\bar{F}(\rho,\Phi,\sigma^\prime,\bs{k})\right].%\sim\frac{1}{\Delta_0|\Psi(\bs{k})|}=\frac{\xi}{|\Psi(\bs{k})|}
\end{align}
It is noted that $\tilde{D},~C>0$ due to $h>0$.
The azimuthal component of the current density is written as
\begin{align}
	j_\Phi(\bs{r})&=-4|e|N_0\pi T\sum_{n=0}^{\infty}\int\frac{d\Omega}{4\pi}v_F\sin\theta\sin(\phi-\Phi) \mathrm{Im}g(\hat{\bs{k}},\bs{r},\omega_n). 
\end{align}
In order to calculate the current density, we perform the sum over the Matsubara frequencies as 
\begin{align}
	-T\sin\theta\sin(\phi-\Phi)\sum_{n=1}^\infty\mathrm{Im}g(\rho,\Phi,\bs{k},i\omega_n)&=\sum_{n=1}^\infty\frac{T\sin\theta\sin(\phi-\Phi)\rho C^{-1}D}{(i\omega_n-\rho D-iC^{-1})(i\omega_n+\rho D-iC^{-1})}\\
				      &=\frac{C^{-1}}{4}\sin\theta\sin(\phi-\Phi)
	\mathrm{Re}\left[\tanh\frac{1}{2T}\left(-\rho D+iC^{-1}\right)\right]
				    \\&\quad+\frac{1}{\pi}\int_0^\infty\frac{\sin^2(\phi-\Phi)\rho C^{-1}\tilde{D}z}{\{(z+\rho D)^2+C^{-2}\}\{(z-\rho D)^2+C^{-2}\}}\tanh\frac{z}{2T}dz.
\end{align}
The second term is bounded from above as
\begin{align}
				      &\quad\frac{1}{\pi}\int_0^\infty\frac{\sin^2(\phi-\Phi)\rho C^{-1}\tilde{D}z}{\{(z+\rho D)^2+C^{-2}\}\{(z-\rho D)^2+C^{-2}\}}\tanh\frac{z}{2T}dz\\
				      &\le\frac{1}{\pi}\int_0^\infty\frac{\sin^2(\phi-\Phi)\rho C^{-1}\tilde{D}z}{\{(z+\rho D)^2+C^{-2}\}\{(z-\rho D)^2+C^{-2}\}}dz
				    \\&=\frac{1}{4\pi}\sin\theta\sin(\phi-\Phi)\int_{-\rho D}^{\rho D}\frac{C^{-1}}{z^2+C^{-2}}dz=2\sin\theta\sin(\phi-\Phi)\tan^{-1}\left(\frac{\rho D}{C^{-1}}\right).
\end{align}
From this inequality, we obtain
\begin{align}
	&\quad-T\sin\theta\sin(\phi-\Phi)\sum_{n=1}^\infty\mathrm{Im}g(\rho,\Phi,\bs{k},i\omega_n)
	\\&\le\frac{C^{-1}}{4}\sin\theta\sin(\phi-\Phi)\mathrm{Re}\left[\tanh\frac{1}{2T}\left(-\rho D+iC^{-1}\right)\right]+2\sin\theta\sin(\phi-\Phi)\tan^{-1}\left(\frac{\rho D}{C^{-1}}\right)
	\\&\simeq\sin^2(\phi-\Phi)\left[-\frac{C^{-1}}{8T}+\frac{2}{C^{-1}}\right]\rho\tilde{D}+O(\rho^2).
\end{align}
Therefore, the vortex current at $\rho\ll\xi$ and
$T\ll\Delta$ is bounded from above as follows:
\begin{align}
	j_\Phi(\rho)&\le4|e|N_0\pi v_F\int\frac{d\Omega}{4\pi}\sin^2(\phi-\Phi)\left[-\frac{C^{-1}}{8T}+\frac{2}{C^{-1}}\right]\rho\tilde{D}.\label{jseq-1}
\end{align}
On the other hand, in the case of $s_\theta=1$ or deep inside the SC, the current density is given by
\begin{align}
	j_\Phi(\rho)&=4|e|N_0\pi v_F\int\frac{d\Omega}{4\pi}\sin\theta\sin(\phi-\Phi)\frac{C^{-1}}{2}\tanh\left(\frac{\rho D}{2T}\right)\\
	      &\simeq4|e|N_0\pi v_F\int\frac{d\Omega}{4\pi}\sin^2(\phi-\Phi)\frac{C^{-1}}{4T}\rho\tilde{D}+O(\rho^2),\label{jseq1}
\end{align}
\end{widetext}
where $N_0$ is the density of state in the normal state.
These equations \eqref{jseq-1} and \eqref{jseq1}
show that the vortex current is reversed
near the surface when $s_\theta=-1$.

The LDOS is written as
\begin{align}
	\frac{N(E,\rho)}{N_0}&=-\lim_{\delta\rightarrow0}\int\frac{d\Omega}{4\pi}\mathrm{Re}g(\bs{k},\bs{r},E+i\delta).
\end{align}
From Eq.~\eqref{fexpand}, the LDOS is calculated as
\begin{align}
	\frac{N(E,\rho)}{N_0}&=-\lim_{\delta\rightarrow0}\int\frac{d\Omega}{4\pi}\mathrm{Re}\frac{\rho D+E+i\delta}{iC^{-1}-\rho D-E-i\delta}
			   \\&=\int\frac{d\Omega}{4\pi}\frac{(\rho D+E)^2}{(\rho D+E)^2+C^{-2}}\le1.
\end{align}
Therefore, the LDOS is
suppressed significantly at $\rho\ll\xi$ and $E\ll|\Delta|$ and equals zero especially at $\rho=0$ and $E=0$.
These results are consistent with numerical results for the
$p_z$-wave SC in the main texts.
%



